Single-Network Whole-Body Pose Estimation

We present the first single-network approach for 2D~whole-body pose estimation, which entails simultaneous localization of body, face, hands, and feet keypoints. Due to the bottom-up formulation, our method maintains constant real-time performance regardless of the number of people in the image. The network is trained in a single stage using multi-task learning, through an improved architecture which can handle scale differences between body/foot and face/hand keypoints. Our approach considerably improves upon OpenPose~\cite{cao2018openpose}, the only work so far capable of whole-body pose estimation, both in terms of speed and global accuracy. Unlike OpenPose, our method does not need to run an additional network for each hand and face candidate, making it substantially faster for multi-person scenarios. This work directly results in a reduction of computational complexity for applications that require 2D whole-body information (e.g., VR/AR, re-targeting). In addition, it yields higher accuracy, especially for occluded, blurry, and low resolution faces and hands. For code, trained models, and validation benchmarks, visit our project page: https://github.com/CMU-Perceptual-Computing-Lab/openpose_train.

==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/0_abstract.tex <==
We present the first single-network approach for 2D~whole-body pose estimation, which entails simultaneous localization of body, face, hands, and feet keypoints. Due to the bottom-up formulation, our method maintains constant real-time performance regardless of the number of people in the image. The network is trained in a single stage using multi-task learning, through an improved architecture which can handle scale differences between body/foot and face/hand keypoints. Our approach considerably improves upon OpenPose~\cite{cao2018openpose}, the only work so far capable of whole-body pose estimation, both in terms of speed and global accuracy. Unlike \cite{cao2018openpose}, our method does not need to run an additional network for each hand and face candidate, making it substantially faster for multi-person scenarios. This work directly results in a reduction of computational complexity for applications that require 2D whole-body information (e.g., VR/AR, re-targeting). In addition, it yields higher accuracy, especially for occluded, blurry, and low resolution faces and hands. For code, trained models, and validation benchmarks, visit our project page\footnote{\url{https://github.com/CMU-Perceptual-Computing-Lab/openpose_train}}.


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/0_teaser.tex <==
% \begin{figure}[t]
%     \centering
    \includegraphics[width=1\linewidth]{figures/teaser/teaser_final.jpg}
    % \begin{subfigure}[t]{1\textwidth}
    % \begin{subfigure}[t]{0.499\textwidth}
    % \includegraphics[width=1\linewidth]{figures/teaser/teaser_OP.png}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.499\textwidth}
    % \includegraphics[width=1\linewidth]{figures/teaser/teaser_our.png}
    % \end{subfigure}
    % \end{subfigure}
    \captionof{figure}{We present the first single-network approach for whole-body pose estimation, with real-time performance independent of the number of people in the image. Our work builds upon the current state-of-the-art OpenPose~\cite{cao2018openpose}, boosting considerably its run-time performance while simultaneously improving slightly on the keypoint accuracy.} \label{fig:teaser}
% \end{figure}


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/1_introduction.tex <==
\section{Introduction}
Human keypoint estimation has been an open problem for decades in the research community. Initially, efforts were focused on facial alignment (i.e., face keypoint detection)~\cite{asthana2014incremental, ranjan2019hyperface, saragih2009face, zhang2016joint, xiong2013supervised, zhang2016learning}, and later evolved into single and multi-person human pose estimation in-the-wild, including body and foot keypoints~\cite{Andriluka2010, belagiannis2017recurrent, cao2017realtime, chen2017cascaded, Dantone2013}. A more recent and challenging problem has targeted hand keypoint detection~\cite{simon2017hand, sridhar2013interactive, zimmermann2017learning}. Therefore, the next logical step is the integration of all of these keypoint detection tasks within the same algorithm, leading to ``whole-body" or ``full-body" (body, face, hand, and foot) pose estimation~\cite{alp2018densepose, cao2018openpose}.

% There are several applications that can immediately take advantage of whole-body keypoint detection, such as %human
% re-targeting and 3D human keypoint and mesh reconstruction~\cite{Recycle-GAN, chan2018everybody, joo2018total, panteleris2017using, xiang2018monocular}. In general, almost any method that uses body information could also %directly
% benefit from face, hand, and foot detection, including person re-identification, tracking, and action recognition%, or AR/VR avatar reconstruction
% ~\cite{gui2018teaching, mehta2017vnect, raaj2018efficient, qian2017pose}. 

There are several applications that can immediately take advantage of whole-body keypoint detection, including augmented reality, virtual reality, medical applications, and sports analytics. Whole-body keypoint detection can also provide more subtle cues for re-targeting, 3D human keypoint and mesh reconstruction~\cite{Recycle-GAN, chan2018everybody, joo2018total, panteleris2017using, xiang2018monocular}, person re-identification, tracking, and action recognition%, or AR/VR avatar reconstruction
~\cite{gui2018teaching, mehta2017vnect, raaj2018efficient, qian2017pose}. Despite these needs, the only existing method providing whole-body pose estimation is the prior version of OpenPose~\cite{cao2018openpose}, which follows a multi-stage approach. First, all body poses are obtained from an input image in a bottom-up fashion~\cite{cao2017realtime} and then additional face and hand keypoint detectors are run for each detected person~\cite{simon2017hand}.
As a multi-network approach, it directly uses the existing body, face, and hand keypoint detection algorithms. However, it suffers from the issue of early commitment: there is no recourse to recovery if the body-only detector fails, especially during partial visibility when only the face or hand are visible in the image. In addition, its run-time is proportional to the number of people in the image, making whole-body pose estimation prohibitively expensive for multi-person and real-time applications. A single-stage method, estimating whole-body poses of multiple people in a single pass, would be more attractive as it would yield a fixed inference run-time, independent of the number of people in the scene. %This method would be analogous to~\cite{cao2017realtime} for the body-only case. %\footnote{In the body-only keypoint estimation area, a single-stage method~\cite{cao2017realtime} is called bottom-up approach where 2D keypoints of multiple people are estimated at once, and then assemble them into full whole-body poses for all people. Our paper pursue the similar goal, yet including faces and hands together}. %This type of approach would directly predict all the keypoints at once, and then assemble them into full whole-body poses for all people. This distinction between single and multi-network approaches is analogous to the distinction between bottom-up and top-down methods for body-only pose estimation. We avoid re-using those terms for simplicity.

Unfortunately, there is an inherent scale difference between body/foot and face/hand keypoints.
% Body and foot detection
The former require a large receptive field to learn the complex interactions across people (contact, occlusion, limb articulation), while the latter require %a smaller receptive field but greater
higher image resolution. Since the foot pose is highly dependent on that of the body, unlike face and hands, its desirable scale is consistent with that of the body. Moreover, the scale issue has two critical consequences. First, datasets with full-body annotations in-the-wild do not currently exist, since the characteristics of each set of keypoints result in different kinds of datasets. Body datasets predominantly contain images with multiple people, usually resulting in fairly low face and hand resolution, while face and hand datasets mostly contain images with a single, cropped face or hand. Secondly, the architecture design of a single-network model must differ from that of the state-of-the-art keypoint detectors in order to offer high-resolution and a larger receptive field, while simultaneously improving the inference run-time of multi-network approaches.

To overcome the dataset problem, we resort to multi-task learning (MTL), a classic machine learning technique~\cite{girshick2015fast, misra2016cross, zhang2014facial} where related learning tasks are solved simultaneously by exploiting commonalities and differences across them. Previously, MTL has been successful in training a combined body-foot keypoint detector~\cite{cao2018openpose}. Nevertheless, it does not generalize to whole-body estimation because of the underlying scale problem. Therefore, the major contributions of this paper are summarized as follows:
\begin{itemize}[noitemsep]
    \item \textbf{Novelty:} We present an MTL approach combined with an improved architecture design to train a unified model for various keypoint detection tasks each with different scale characteristics. %We apply this MTL technique with an updated model architecture design, and demonstrate
    This results in the \textit{first} single-network approach for whole-body multi-person pose estimation. %This method maintains constant real-time performance regardless of the number of people detected, and state-of-the-art accuracy on each individual annotation task (body, face, hand, and foot).
    \item \textbf{Speed:}
    %Our method demonstrates a considerably faster inference runtime than the state-of-the-art (OpenPose~\cite{cao2018openpose}).
    At test time, our single-network approach provides a constant real-time inference regardless of the number of people detected, and it is approximately $n$ times faster than the state-of-the-art (OpenPose~\cite{cao2018openpose}) for images with $n$ people. In addition, it is trained in a single stage, rather than requiring independent network training for each individual task. This reduces the total training time approximately by one-half.
    \item \textbf{Accuracy:} Our approach also yields higher accuracy than that of the previous OpenPose, especially for face and hand keypoint detection, generalizing better to occluded, blurry, and low resolution faces and hands.
    % common in-the-wild challenges (e.g., occluded, blurry, and low resolution faces and hands).
    % In addition, it maintains similar accuracy for body and foot detection. % compared to the the state-of-the-art.%  especially for in-the-wild benchmarks. In addition, body and foot detection accuracy remains similar to that of the dedicated body-foot OpenPose detector.
\end{itemize}


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/2_related_work.tex <==
\section{Related Work}
\textbf{Face Keypoint Detection:} Also referred in literature as landmark detection or face alignment, it has a long history in computer vision and many approaches have been proposed to tackle it. These approaches are broadly divisible into two categories:
template fitting~\cite{asthana2014incremental, kazemi2014one, saragih2009face, xiong2013supervised, zhu2015face} and regression-based
% methods~\cite{cao2018openpose, ranjan2019hyperface, zhang2016joint, zhang2016learning}.
methods~\cite{ranjan2019hyperface, zhang2016joint, zhang2016learning}.
Template fitting methods build face templates to fit input images, usually exploiting a cascade of regression functions.
% State-of-the-art
Regression methods,
on the other hand,
are based on Convolutional Neural Networks (CNNs) and usually apply convolutional heatmap regression. They operate in a similar fashion to that of body pose estimation.



\textbf{Body Keypoint Estimation:}
With the face alignment problem solved, efforts moved towards single-person pose estimation. The initial approaches performed inference over both local observations on body parts and their spatial dependencies, either based on tree-structured graphical models~\cite{Andriluka2010,fh2005pictorial,pishchulin2013poselet,ramanan2005strike,yang2013articulated} %johnson2010clustered,
or non-tree models~\cite{Dantone2013,karlinsky2012using,lan2005beyond,sigal2006measure,wang2008multiple}.
The popularity of CNNs and the release of massive annotated datasets (COCO~\cite{lin2014microsoft} and MPII~\cite{andriluka20142d})
% significantly boost the accuracy
imparted significant boost in the accuracy
of single-person estimation~\cite{belagiannis2017recurrent,chen2017adversarial,chu2017multi,Ke_2018_ECCV,newell2016stacked,tang2018deeply,wei2016cpm,yang2017learning}, %bulat2016human,tompson2014joint,ouyang2014multi,Chen_NIPS14,toshev2014deeppose,tompson2014efficient,
and %eventually
have enabled multi-person estimation. The latter is traditionally divided into top-down~\cite{chen2017cascaded,fang2017rmpe,gkioxari2014using,he2017mask,iqbal2016multi,papandreou2017towards,pishchulin2012articulated,xiao2018simple} %sun2011articulated,
and bottom-up~\cite{cao2017realtime, newell2017associative, nie2018ppn, papandreou2018personlab, pishchulin2015deepcut} %cao2017realtime, insafutdinov2016deepercut, insafutdinov2017arttrack,
approaches.

\textbf{Foot Keypoint Estimation:}
Cao~\etal~\cite{cao2018openpose} released the first foot dataset, with annotations on a subset of images from the COCO dataset.
They also trained the first combined body-foot keypoint detector
% They also trained the first foot keypoint detector with a network that combined the body keypoints from COCO and their foot keypoints,
by applying a naive multi-task learning technique. %and masking out the channels corresponding to the non-labeled keypoints from each dataset.
Our method is an extension of this work, mitigating its limitations and enabling it to generalize to both large-scale body and foot keypoints as well as the more subtle face and hand keypoints. %, as we will discuss in Sec.~\ref{sec:method}.






\begin{figure*}[t]%[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/arch_inkscape.pdf}
    % \includegraphics[width=1\linewidth]{figures/arch_inkscape.png}
    %     \vspace{-22pt}
    \caption{Overall pipeline.
    (a)~An RGB image is taken as input.
    (b,c)~Architecture of the %end-to-end
    whole-body pose estimation network, consisting of multiple stages predicting refined PAFs ($\mathbf{L}$) and confidence maps ($\mathbf{S}$) for body, face, hand and foot.
    It is trained end-to-end with a multi-task loss that combines the losses of each individual keypoint annotation task.    %   During training, we
%   randomly
% %   selectively
%   alternate between whole-body part sets, each with its own unique augmentation characteristics, while masking out the back-propagation losses from unlabeled keypoints. %, emulating a Multi-Task-Learning strategy.
    Each \textit{Conv Layer}, $\mathrm{C}$,  corresponds to a Convolution-PReLU sequence.
   (d)~At test time, the most refined PAFs and confidence maps are resized to increase the accuracy. %output by the network
   (e)~The parsing algorithm uses the PAFs to find all the whole-body parts belonging to the same person using bipartite matching.
   (f)~The final whole-body poses are returned for all the people in the image.
   }
   \label{fig:architecture}
    % \vspace{-10pt}
    % \vspace{-13pt}
\end{figure*}



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/architecture.png}
%     \caption{Architecture of the end-to-end fully body network, consisting of multiple stages predicting and refining Part Affinity Fields $\rho$, producing heatmaps $\mathbf{L}$, which incorporate {$L_B,L_F,L_H,L_f$} body, face, hand and foot connections. $\mathbf{S}$ is then passed to a network jointly predicting confidence maps $\phi$, producing heatmaps $\mathbf{S}$ for all keypoints in a single stage. During training, we selectively alternative between body part sets, each with it's own unique augmentation characteristics, by masking out relevant  $\mathbf{S}$/ $\mathbf{L}$ heatmaps, emulating a Multi-Task-Learning strategy.}
%     \label{fig:architecture}
% \end{figure}


\textbf{Hand Keypoint Detection:}
With the exciting improvements in face and %multi-person
body estimation, recent research is targeting hand keypoint detection. However, its manual annotation is extremely challenging and expensive due to heavy self-occlusion~\cite{simon2017hand}. As a result, large hand keypoint datasets do not exist in-the-wild. To alleviate this problem, early work %on hand detection
is based on depth information~\cite{oikonomidis2012tracking, sharp2015accurate, sridhar2015fast, sridhar2013interactive}, % tzionas2016capturing, ye2016spatial
but is limited to indoor scenarios. %due to the depth sensor limitations.
% However, these methods are limited to indoor scenarios. %due to the depth sensor limitations.
Most of the work in RGB-based hand estimation is focused on 3D estimation~\cite{cai2018weakly, iqbal2018hand, mueller2018ganerated, zimmermann2017learning}, primarily based on fitting complex 3D models with strong priors. In the 2D RGB domain, Simon \textit{et al.}~\cite{simon2017hand} exploit multi-view bootstrapping to create a hand keypoint dataset and train a 2D RGB-based hand detector. First, a naive detector is trained on a small subset of manually labeled annotations.
Next, this detector is applied in a 30-camera multi-view dome structure~\cite{Joo_2015_ICCV, joo2018total} to obtain new annotations based on 3D reconstruction.
% Next, its accuracy is ``bootstrapped" by re-projecting the initial hand detector results into a 30-camera multi-view dome structure~\cite{Joo_2015_ICCV, joo2018total} to obtain new annotations.
%This process is repeated to convergence.
Unfortunately, most of the methods have only demonstrated results in controlled lab environments. % due to the lack of available in-the-wild datasets. %hand keypoint datasets. %, and only OpenPose~\cite{cao2018openpose} seems to provide decent results for in-the-wild 2D hand pose estimation.



\textbf{Whole-Body Keypoint Detection:}
OpenPose~\cite{cao2018openpose, cao2017realtime, simon2017hand} is the only known work able to provide all body, face, hand, and foot keypoints in 2D. It operates in a multi-network fashion. First, it detects the body and foot keypoints based on~\cite{cao2017realtime, wei2016cpm}. Then, it approximates the face and hand bounding boxes based on the body keypoints, and applies a keypoint detection network for each subsequent face and hand candidate~\cite{simon2017hand}. Recent work is also targeting 3D mesh reconstruction~\cite{joo2018total, kanazawa2018end}, usually leveraging the lack of 3D datasets with the existing 2D datasets and detectors, or reconstructing the 3D surface of the human body from denser 2D human annotations~\cite{alp2018densepose}.



\textbf{Multi-Task Learning:}
To overcome the problems of state-of-the-art whole-body pose estimation, we aim to apply multi-task learning (MTL) to train a single whole-body estimation model out of the four different tasks: body, face, hand, and foot detection. MTL applied to deep learning can be split into soft and hard parameter sharing of hidden layers. In soft parameter sharing, each task has its own model, but the distance between the parameters is regularized to encourage them to be similar between models~\cite{duong2015low, yang2016trace}. Hard parameter sharing is the most commonly used MTL approach in computer vision, applied in many applications, such as facial alignment~\cite{zhang2014facial} or surface normal prediction~\cite{misra2016cross}. Particularly, it has had a critical impact on object detection, where popular approaches such as Fast R-CNN~\cite{girshick2015fast} exploit MTL to merge all previously independent object detection tasks into a single and improved detector. It considerably improved training and testing speeds as well as detection accuracy. Analogous to Fast R-CNN, our work brings together multiple and independent keypoint detection tasks into a unified framework. See~\cite{ruder2017overview} for a more detailed survey of multi-task learning literature.


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/3_method.tex <==
\section{Method}\label{sec:method}
Our system follows a streamlined approach, using an RGB image to generate a set of whole-body human keypoints for each person detected. This global pipeline is illustrated in Fig.~\ref{fig:architecture}. The extracted keypoints contain information from the face, torso, arms, hands, legs, and feet.
% We could apply our Multi-Task Learning (MTL) method to any body-only keypoint estimation technique.
The network architecture of the proposed whole-body keypoint detector can be based on any state-of-the-art body-only keypoint detector.
% We can train our whole-body keypoint detector based on any state-of-the-art body-only keypoint detector.
For a fair comparison of our results with previous versions of OpenPose~\cite{cao2018openpose, cao2017realtime, simon2017hand}, we reuse its Part Affinity Field (PAF) network architecture.



\subsection{PAF-based Body Pose Estimation}
Here, we review the main details of the PAF-based method. We refer the reader to~\cite{cao2017realtime} for a full description. % of the approach. %, so the reader can later understand the required changes to enable whole-body estimation. 
This approach iteratively predicts Part Affinity Fields (PAFs), which encode part-to-part associations, and detection confidence maps. Each PAF is defined as a 2D orientation vector that points from one keypoint to another. %This vector encodes the direction that points from one to the other.
The input image $I$ is initially analyzed by a convolutional network (pre-trained on VGG-19~\cite{simonyan2014very}), generating a set of feature maps $\mathbf{F}$. Next, $\mathbf{F}$ is fed into the first stage $\phi^{(1)}$ of the network $\phi$, which predicts a set of PAFs $\mathbf{L}^{(1)}$. For each subsequent stage $i$, the PAFs of the previous stage $\mathbf{L}^{(t-1)}$ are concatenated to $\mathbf{F}$ and refined to produce $\mathbf{L}^{(t)}$. After $N$ stages, we obtain the final set of PAF channels $\mathbf{L} = \mathbf{L}^{(N)}$. Then, $\mathbf{F}$ and $\mathbf{L}$ are concatenated and fed into a network $\rho$, which predicts the keypoint confidence maps $\mathbf{S}$, i.e.,
%\vspace{-5pt}
%vspace{-5pt}
\begin{gather}
\mathbf{L}^{(1)}=\phi^{(1)}\left(\mathbf{F}\right),
\\
\mathbf{L}^{(t)}=\phi^{(t)}\left(\mathbf{F},\mathbf{L}^{(t-1)}\right),\:\text{\ensuremath{\forall}}~2\leq t\leq N,
\\
\mathbf{L}=\mathbf{L}^{(N)},
\\
\mathbf{S}=\rho\left(\mathbf{F},\mathbf{L}\right).
\end{gather}

An $\ell$2 loss function is applied at the end of each stage, which compares the estimated predictions and the groundtruth maps ($\mathbf S^*$) and fields ($\mathbf L^*$) for each pixel ($p$) on each confidence map ($c$) and PAF ($f$) channel:
\begin{gather}
f_{\mathbf{L}}=\sum_{f=1}^F\sum_{p}\left(W_i(p) \cdot \Vert\mathbf{L}_f(p)-\mathbf{L}_f^*(p)\Vert_2^2\right),
\\
f_{\mathbf{S}}=\sum_{c=1}^{C}\sum_{p}\left(W_i(p) \cdot \Vert\mathbf{S}_c(p)-\mathbf{S}_c^*(p)\Vert_2^2\right),
\end{gather}
where $C$ and $F$ are the number of stages for confidence map and PAF prediction, and $W$ is a binary mask with $W_i(p)$=0 when an annotation is missing at a pixel %location
$p$ for a particular confidence map or PAF channel $i$. Non-maximum suppression is performed on the confidence maps to obtain a discrete set of body part candidate locations. Finally, bipartite graph matching~\cite{west1996introduction} is used to assemble the connections that share the same part detection candidates into full-body poses for each person in the image.




\subsection{Whole-Body Pose Estimation}
We want whole-body pose estimation to be accurate but also fast. Training an individual PAF-based network to predict each individual set of keypoints would achieve the first goal, but would also be computationally inefficient. Instead, we extend the body-only PAF framework to whole-body pose estimation, making various modifications to the training approach and network architecture.

\textbf{Multi-task learning training:}
We modify the definition of the keypoint confidence maps $\mathbf{S}$ as the concatenation of the confidence maps: body $S_B$, face $S_F$, hand $S_H$, and foot $S_O$. Analogously, the set of PAFs at stage $t$, $\mathbf{L}^{(t)}$, is defined as the concatenation of the PAFs: body $\mathbf{L}_B^{(t)}$, face $\mathbf{L}_F^{(t)}$, hand $\mathbf{L}_H^{(t)}$, and foot $\mathbf{L}_O^{(t)}$.
%and all keypoints had similar characteristics, we could directly train this model.
An interconnection between the different annotation tasks must %also
be created in order to allow the different
% body, face, hand, and foot
set of
keypoints of the same person to be assembled together. For instance, we join the body and foot keypoints through the ankle keypoint, which is annotated in both datasets. Analogously, the wrists connect the body and hand keypoints, while the eyes relate body and face.
% In this particular case, the ankle keypoint is labeled in both body and foot datasets, and analogously the wrist keypoint is labeled for body and hand annotations. Thus, no extra connections are required for those / ankle and wrist. For the face dataset, we train the definition of eye from the body datasets with the averaged point between the multiple eyelid keypoints annotated in the face datasets. This way, we can create new PAFs $L_{BF}^{(i)}$ between the body and face keypoints.
% Shoulders to join COCO and MPII datasets.
The rest of the pipeline (non-maximum suppression over confidence maps and bipartite matching to assemble full people) is left intact.
As opposed to having a dedicated network for each keypoint annotation task, all the keypoints are now defined within the same model architecture. This is an extreme version of hard parameter sharing, in which only the final layer is task-specific.
% If there were a whole-body dataset as big and diverse as the COCO~\cite{lin2014microsoft} body dataset, we could directly train a combined model and multi-task learning would not be required.
% If we had a whole-body dataset as big and diverse as the COCO~\cite{lin2014microsoft} body dataset,
% multi-task learning would not be required.
% %and all keypoints had similar characteristics, we could directly train this model.
% If we had a whole-body dataset, we could directly train this model.



% \subsubsection{Whole-Body Training via Naive Multi-Task Learning}
\textbf{Balanced dataset-based probability ratio:}
If we had a whole-body dataset, we could train a combined model following the body-only training approach. Unfortunately, each available dataset only contains annotations for a subset of keypoints.
To overcome the lack of a combined dataset, we follow the probability ratio idea of the single-network body-foot detector of Cao~\etal~\cite{cao2018openpose}, which was trained from body-only and body-foot datasets.
% We initially train a detector following the ideas of the combined body-foot detector of Cao~\etal~\cite{cao2018openpose}. To overcome the lack of a combined dataset, batches
Batches
of images are randomly picked from each available dataset, and the losses for the confidence map and PAF channels associated to non-labeled keypoints are masked out. I.e., their binary mask $W_i(p)$ is set to 0. Abusing notation, the probability ratio $P^d$ is defined as the probability of picking the next annotated batch of images from the dataset $d$. This probability is distributed across the different datasets depending on the number of images in each dataset. % As pointed out in~\cite{cao2018openpose}, $P^d$ must be applied to a whole batch, rather than to single images. Otherwise, the effective batch size for each annotation task would differ. For instance, if we assume a batch size of 10 images and a 10\% probability of selecting an image from the foot dataset, on average only 1 image per batch would contain foot annotations. This is approximately equivalent to applying a batch size of 1 for foot keypoint training, yielding an extremely low accuracy.
% The L2 loss is re-defined as follows:
% \begin{gather}
% f_{\mathbf{L}}=\sum_{f=1}^F\sum_{p}\left(W_f(p) \cdot \Vert\mathbf{L}_f(p)-\mathbf{L}_f^*(p)\Vert_2^2\right)
% \\
% f_{\mathbf{S}}=\sum_{c=1}^{C}\sum_{p}\left(W_c(p) \cdot \Vert\mathbf{S}_c(p)-\mathbf{S}_c^*(p)\Vert_2^2\right)
% \end{gather}
% where the updated $W$ is a binary mask with $W_i(p) = 0$ when an annotation is missing at a pixel location $p$ for a confidence map or PAF channel $i$.
% When applied to similar datasets
When applied to keypoints with similar scale properties (e.g., body and foot~\cite{cao2018openpose}), it results in a robust keypoint detector. However,  it does not converge when applied to whole-body estimation, which now includes face and hand keypoints. Additionally, the accuracy of the body and foot detectors is considerably reduced.
% \subsubsection{Whole-Body Training via Smart Multi-Task Learning}
Solving the face and hand convergence problem would be then possible through
a deeper analysis of the properties and differences of each set of keypoints.
% further refinement of the training methodology and datasets.

% \begin{figure*}[t]
\begin{figure}[t]
\centering
    % \begin{subfigure}[t]{0.325\textwidth}
    \begin{subfigure}[t]{0.325\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/hand_480.jpg}
        \caption{}
    \end{subfigure}
    % \begin{subfigure}[t]{0.325\textwidth}
    \begin{subfigure}[t]{0.325\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/body.jpg}
        \caption{}
    \end{subfigure}
    % \begin{subfigure}[t]{0.325\textwidth}
    \begin{subfigure}[t]{0.325\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/face.jpg}
        \caption{}
    \end{subfigure}
    % \vspace{-5pt}
   \caption{Different kinds of datasets for each set of keypoints present different properties (number of people, occlusion, person scale, etc.).
   We show typical examples from the hand (left), body (center), and face (right) datasets.
   }
    % \vspace{-10pt}
\label{fig:dataset_examples}
\end{figure}
% \end{figure*}

\textbf{Dataset-based augmentation:}
% Solving the face and hand convergence problem requires
% a deeper look to the datasets.
% resolving several dataset issues.
% understanding
% the
There is an inherent scale difference between body/foot and face/hand keypoints,
which results in different kinds of datasets for each set of keypoints. Body datasets predominately contain images with multiple people and low face and hand resolution; face datasets focus on images with a single person or cropped face; whereas hand datasets usually contain images with a single full-body person. Fig.~\ref{fig:dataset_examples} shows typical examples from each dataset.
To solve this problem, augmentation parameters are varied for each set of keypoints. For instance, the minimum possible scale for face datasets is reduced during data augmentation to expose our model to small faces, % during training,
to simulate reality of the `wild' environments. Oppositely, the maximum scale for hand datasets is increased so that full-sized hands appear more frequently, allowing the network to generalize to high resolution hands.

\textbf{Overfitting:}
Using the above ideas, the face and hand detectors converge and allow us to build an initial whole-body pose detector.
%After solving these issues, the face and hand detectors finally converge and we can build a working whole-body pose detector.
However, we observe a large degree of over-fitting on some validation sets, particularly in the face and lab-recorded datasets. Even though the initial probability ratio $P^d$ is evenly distributed depending on the number of images in each dataset, the data complexity of these datasets is lower than the complexity of the challenging multi-person and in-the-wild datasets. In addition, the range of possible facial gestures is much smaller than the number of possible body and hand poses. Thus, the probability ratio of picking a batch from one of the face and lab-recorded datasets must be additionally reduced. Empirically, we fine-tune the probability ratios between datasets so that the validation accuracy on each converges at the same pace.

\textbf{High false positive rate:}
Face, hand, and foot keypoints present a high false positive rate producing a ``ghosting" effect on their respective confidence map and PAF channels. Visually, this means that these channels are outputting a non-zero value in regions that do not contain people. To mitigate this issue,
% we train these sets of keypoints in the COCO dataset for the regions of the image without people, by maintaining their binary mask $W_i(p)$ enabled.
their binary mask $W_i(p)$
is re-enabled in the COCO dataset for image regions with no people. Furthermore, we complement training with an additional dataset consisting of COCO images without any people.

\textbf{Further refinement:}
Face and hand datasets do not necessarily annotate all the people that appear in each image. % They were initially built for bounding-box single-face and single-hand detectors that assumed a given bounding box with only an instance.
We apply Mask R-CNN~\cite{he2017mask} to mask out the regions of the image with non-labeled people. %, by setting their binary mask to 0.
In addition, the pixel localization precision of the face and hand keypoint detectors remains low. To moderately improve it, we reduce the radius of the Gaussian distribution used to generate the groundtruth of their confidence map channels. %This reduction could lead to an increase of the false negative rate. for those channels. Their binary mask $W$ is greater than 1 to balance the weight across all keypoints.

\textbf{Shallow whole-body detector:}
At this point, we can build a working whole-body pose detector.
The inference run-time of this refined detector matches that of running body-foot in~\cite{cao2018openpose}. However, it still suffers from two main issues. On the one hand, the body and foot accuracy considerably decreases compared to its standalone analog (i.e., the body-foot detector from Cao~\etal~\cite{cao2018openpose}). The complexity of the network output has increased from predicting 25 to 135 keypoints (and their corresponding PAFs). The network has to compress about 5 times more information with the same number of parameters, reducing the accuracy of each individual part. On the other hand, face and hand detection accuracy appear relatively similar to that of Cao~\etal~\cite{cao2018openpose} in the benchmarks, but the qualitative results show that their pixel localization precision remains low. This is due to the reuse of same network as that used in body-only pose estimation which has low input resolution. Face and hand detection requires a network with higher resolution to provide results with high pixel localization precision. This initial detector is defined as ``Shallow whole-body" in Sec.~\ref{sec:evaluation}.

% \subsubsection{Whole-Body Training via Smarter Multi-Task Learning}
\textbf{Improved network architecture:}
To match the accuracy of the body-only detector and solve the resolution issue of face and hand, the whole-body network architecture must diverge from that of Cao~\etal~\cite{cao2018openpose}. It must still maintain a large receptive field for accurate body detection but also offer high-resolution maps for precise face and hand keypoint detection. Additionally, its inference run-time should remain similar to or improve upon that of its analogous multi-stage whole-body detector. Our final model architecture, refined for whole-body estimation and shown in Fig.~\ref{fig:architecture}, differs from the original baseline in the following details:
\begin{itemize}[noitemsep]
    \item The network input resolution is increased to considerably improve face and hand precision. Unfortunately, this implicitly reduces the effective receptive field (further reducing body accuracy). % and runtime performance.
    \item The number of convolutional blocks in each PAF stage is increased to recover the effective receptive field that was previously reduced. %However, it further decreases the runtime performance.
    \item The width of each convolutional layer in the last PAF stage is increased to improve the overall accuracy, enabling our model to match the body accuracy of the standalone body detector. %The runtime performance is reduced again.
    \item The previous solutions considerably increase the overall accuracy of our approach but also harm the training and testing speed. The number of PAF stages is reduced to partially overcome this issue, which only results in a moderate reduction in overall accuracy.
    % The number of PAF stages is reduced to balance the considerable runtime performance drop due to our deeper model. This results in a considerable increase of runtime performance, with only a moderate reduction in overall accuracy.
\end{itemize}

This improved model highly outperforms Cao~\etal~\cite{cao2018openpose} in speed, being approximately $n$ times faster for an image with $n$ people in it. Additionally, it also slightly improves its global accuracy (Secs.~\ref{sec:body_val}, \ref{sec:face_val} and \ref{sec:hand_val}).
% This improved model benefits from higher accuracy and speed compared to that of OpenPose. On one hand, the body accuracy increases (Sec~\ref{sec:body_val}), while the face and hand detection quality is remarkably improved (Sec.~\ref{sec:face_val} and \ref{sec:hand_val}). On the other hand, our method is approximately $p\times$ faster, where $n$ is the number of detected people (Sec.~\ref{sec:runtime_comparison}).
This network is denoted as ``Deep whole-body" in Sec.~\ref{sec:evaluation}.
% This network is denoted as ``Deep whole-body". We show in Sec.~\ref{sec:face_val} and Sec.~\ref{sec:hand_val} that combining all the keypoint detection tasks into a single model considerably help face and hand detection to generalize better. Unfortunately, increasing the network complexity directly results in slower inference time. Our final model runtime performance matches that of running whole-body OpenPose for 1 person (i.e., the time of running the independent body-foot, face, and hand detectors). See Sec.~\ref{sec:runtime_comparison} for a detailed runtime comparison.


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/4_evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}
% We train and evaluate our method on different benchmarks for each set of keypoints. Our approach significantly exceeds the previous state-of-the-art results on face and hand estimation. We also provide a run-time analysis comparison to quantify the efficiency of the system and analyze the main failure cases.

\subsection{Experimental Setup}\label{sec:param_config}
\textbf{Datasets:}
% Following~\cite{cao2018openpose}, w
We train and evaluate our method on different benchmarks for each set of keypoints:
% (1) MPII human multi-person dataset~\cite{andriluka20142d}, which consists of 3844 training and 1758 testing groups of multiple interacting individuals in highly articulated poses with 14 body parts;
% (1) COCO keypoint challenge dataset~\cite{lin2014microsoft}, which requires simultaneously detecting people and localizing 17 body keypoints in each person;
(1)~COCO keypoint % challenge
dataset~\cite{lin2014microsoft} for multi-person body estimation;
(2)~OpenPose foot dataset~\cite{cao2018openpose}, which is a subset of 15k annotations out of the COCO keypoint dataset;
(3)~OpenPose hand dataset~\cite{simon2017hand}, which combines a subset of 1k hand instances manually annotated from MPII~\cite{andriluka20142d} as well as a set of 15k samples automatically annotated on the Dome or Panoptic Studio~\cite{Joo_2017_TPAMI};
(4)~our custom face dataset, consisting of a combination of the CMU Multi-PIE Face~\cite{gross2010multi}, Face Recognition Grand Challenge (FRGC)~\cite{frgc_2010}, and i-bug~\cite{sagonas2016300} datasets;
(5)~the Monocular Total Capture dataset~\cite{xiang2018monocular}, the only available 2D whole-body dataset which has been recorded in the same Panoptic Studio used for the hand dataset. %This dataset should particularly help the PAFs between keypoints of the different annotation tasks. Feedback here: Why? Is this clear for other CV people? It is not for me. %Both this dataset and the hand datasets have been recorded  has also been recorded on the Panoptic Studio~\cite{Joo_2017_TPAMI}, being similar to the hand dataset~\cite{simon2017hand}.
Following the standard COCO multi-person metrics, we report mean Average Precision (AP) and mean Average Recall (AR) for all sets of keypoints. %, both averaged over 10 OKS thresholds. OKS refers to Object Keypoint Similarity, defined by the COCO evaluation guidelines, and is the analog of IoU in object detection. %The official face and hand PCK metrics 


\textbf{Training:} All models are trained using 4-GPU machines, with a batch size of 10 images, Adam optimization, and an initial learning rate of 5e-5. We also decrease the learning rate by a factor of 2 after 200k, 300k, and every additional 60k iterations. We apply random cropping, rotation ($\pm$45$^o$), flipping (50\%), and scale (in the range $[1/3, 1.5]$) augmentation. The scale is modified to $[2/3, 4.5]$ and $[0.5, 4.0]$ for Dome and MPII hand datasets, respectively. The input resolution of the network is set to $480$$\times$$480$ pixels. Similar to~\cite{cao2018openpose}, we maintain VGG-19 as the backbone. The probability of picking an image from each dataset is 76.5\% for COCO, 5\% each for foot and MPII datasets, 0.33\% for each face dataset, 0.5\% for Dome hand, 5\% for MPII hand, 5\% for whole-body data, and 2\% for picking an image with no people in it.

\textbf{Evaluation:} We report both single-scale (image resized to a height of 480 pixels while maintaining the aspect ratio) and multi-scale results
(results averaged from images resized to a height of 960, 720, 480, and 240 pixels).
% (averaging the results at 4 different scales, corresponding to a height of 960, 720, 480, and 240 pixels).



% We experiment with different networks width of each convolutional layer 

% Compared to OpenPose~\cite{cao2018openpose}, our final model training parameters are as follows:
% \begin{enumerate}
%     \item The network input resolution is increased from 368$\times$368 to 480$\times$480.
%     \item The width of each convolutional layer in the last PAF stage is increased from 128 to 256 output channels.
%     \item The number of convolutional blocks per PAF stage is increased from 5 to 8.
%     \item The number of PAF stages is reduced from 5 to 4.
%     \item The probability of picking an image from each dataset is 65\% for COCO, 5\% for foot and MPII, 1\% for CMU Multi-PIE and FRGC, 3\% for i-bug, 2\% for Dome hand, 6\% for MPII hand, 10\% for whole-body data, and 2\% for picking an image with no people in it.
%     \item The default scale data augmentation is in the range $[1/3, 1.5]$. For Dome and MPII hand, the range is modified to $[2/3, 4.5]$ and $[0.5, 4.0]$, respectively.
% \end{enumerate}


\subsection{Ablation Experiments}
Increasing the network resolution is crucial for accurate hand and face detection. Nevertheless, it directly results in slower training and testing speeds. We aim to maximize the accuracy while preserving
% the computational complexity during inference.
a reasonable run-time performance.
Thus, we explore multiple models tuned to maintain the same inference run-time. The final model is selected as the one maximizing the body AP.
Table~\ref{table:self_coco_val} shows the results on the COCO~\cite{lin2014microsoft} validation set. %per computation cost.
% Our final architecture is selected as the one maximizing the body AP.
The most efficient configuration is achieved by increasing the number of convolutional blocks and their width, while reducing the number of stages in order to preserve the speed. %In Table~\ref{table:self_coco_val}, we show self-comparison results on the COCO~\cite{lin2014microsoft} validation set.
% In addition, combining all keypoints into the same network boost face and hand accuracy, but harms body detection. To minimize this problem, our final architecture is selected as the one maximizing the body accuracy. In Table~\ref{table:self_coco_val}, we show self-comparison results on the COCO~\cite{lin2014microsoft} validation set.

%\vspace{-5pt}
\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|c|c|c|c}
    \hline
    \multicolumn{2}{c|}{Method}    & \multirow{2}{*}{AP} & \multirow{2}{*}{AR} & \multirow{2}{*}{APs} & \multirow{2}{*}{ARs} \\
    \cline{1-2}
    \multicolumn{1}{c|}{PAF} & \multicolumn{1}{c|}{CM} & & & & \\
    \hline
    % {\scriptsize N, PAF (1s, 9b, 256w), CM (1s, 9b, 192w)} & XX & XX & 54.2 & 59.7 & 10154 & 120\\ % 1_25BSuperModel11FullVGGFix
    % {\scriptsize N, PAF (1s, 9b, 256w), CM (1s, 9b, 192w)} & XX & XX & 55.2 & 60.3 & 11619 & 120\\ % 2_25BSuperModel11FullVGGDeep
    % {\scriptsize N, PAF (1s, 9b, 256w), CM (1s, 9b, 192w)} & XX & XX & 53.4 & 58.7 & 10548 & 121\\ % 5_25BSuperModel11FullVGGDeepConcat
    % {\scriptsize N, PAF (1s, 9b, 256w), CM (1s, 9b, 192w)} & 66.7 & 71.2 & 57.3 & 62.5 & 10170 & 119\\ % 1_25BSuperModel11FullVGG
    % {\scriptsize DC, PAF (1s, 8b, 256w), CM (1s, 8b, 256w)} & 65.6 & 70.1 & 56.2 & 61.0 & 9414 & 118\\ % 1_25BSuperModel11PreDC
    %
      1s, 10b, \hphantom{000-}256w & 1s, 10b, 256w & 65.8 & 70.3 & 56.1 & 61.1 \\% & 9335 & 116 \\ % 3_25BSuperModel11
    % {\scriptsize PAF (2s, 8b, 128-320w), CM (1s, 5b, 256w)} & 66.0 & 70.5 & 56.4 & 61.7 & XXX & 130 \\ % 3_25BSuperModel21Wider2
      2s, \hphantom{0}8b, 128-288w & 1s, \hphantom{0}8b, 256w & 66.1 & 70.5 & 56.7 & 61.9 \\% & XXX & 121 \\ % 1_25BSuperModel21HM2
      2s, 10b, 128-256w & 1s, 10b, 256w & 66.1 & 70.7 & \textbf{57.0} & \textbf{62.0} \\% & 9993 & 126 \\ % 2_25BSuperModel21deepAndHM
    % {\scriptsize N, PAF (2s, 8b, 128-256w), CM (1s, 8b, 192w)} & 66.8 & 71.2 & 56.9 & 62.1 & 10259 & 118 \\ % 2_25BSuperModel21FullVGG
      3s, \hphantom{0}8b, \hphantom{0}96-256w & 1s, \hphantom{0}8b, 192w & \textbf{66.4} & \textbf{70.9} & 56.9 & 61.9 \\% & 10349 & 120 \\ % 5_25BSuperModel31DeepAndHM
    % {\scriptsize DC, PAF (3s, 6b, 96-256w), CM (1s, 6b, 192w)} & 66.0 & 70.4 & 56.4 & 61.6 & 9597 & 118 \\ % 2_25BSuperModel31PreDC
    % {\scriptsize DC, PAF (3s, 4b, 96-256w), CM (1s, 4b, 192w)} & 65.9 & 70.7 & \textbf{57.2} & \textbf{62.4} \\% & 10139 & 117 \\ % 1_25BSuperModel31PreDCConcat
      4s, \hphantom{0}8b, \hphantom{0}96-256w & 1s, \hphantom{0}8b, 224w & 65.7 & 70.2 & 56.3 & 61.4 \\% & 10656 & 120 \\ % 5_25BSuperModel41
      5s, \hphantom{0}8b, \hphantom{0}64-256w & 1s, \hphantom{0}5b, 256w & 65.5 & 70.1 & 56.7 & 61.8 \\% & XXX & 119 \\ % 2_25BSuperModel
    \hline
    \end{tabular}}
    % \vspace{-10pt}
    \vspace{-5pt}
    \caption{Self-comparison on the body COCO validation set. All models have been tuned to have the same inference run-time. `APs' and `ARs' refer to the single-scale results.
    `PAF' represents the Part Affinity Field network configuration and `CM' the confidence map configuration. `s' refers to the number of stages of refinement, `b' to the number of convolutional blocks per stage, `w' to the number of output channels (or width) of each convolutional layer. All other settings follow Sec.~\ref{sec:param_config}.}
    % \vspace{-15pt}
    % \vspace{-5pt}
    \label{table:self_coco_val}
\end{table}


\subsection{Body and Foot Keypoint Detection Accuracy}\label{sec:body_val}
Once the optimal model %architecture
has been selected, it is trained for whole-body estimation. Table~\ref{table:coco_val} show the accuracy results on the COCO validation set for our 3 different models, as well as the results reported by Cao~\etal~\cite{cao2018openpose}. %As we can see, n
The new deeper architecture slightly increases the accuracy of OpenPose when trained for whole-body estimation. It can also be applied to body-foot estimation, achieving a 1.1\% improvement in accuracy compared to that of Cao~\etal~\cite{cao2018openpose}.
Interestingly, adding face and hand keypoints to the same model results in a considerable decrease of the body detection accuracy by about 5\% for the shallow model when compared to that of \cite{cao2018openpose}. Intuitively, this is due to the fact that we are trying to fit nearly six times as many keypoints into the same network. %By increasing the network depth and input resolution as detailed in Sec.~\ref{sec:method}, while keeping all keypoints, we can mostly overcome this problem, leading to an accuracy drop less than 1\%.
%Our improved architecture outperforms the accuracy of OpenPose 1.1\% when trained only for body-foot detection, and 0.3\% when trained for whole-body estimation. In addition,
The original model might not have enough capacity to handle the additional complexity introduced by the new keypoints.
However, this gap is smaller than 1\% for the improved architecture (deep body-foot vs. deep whole-body). The additional depth helps the network generalize to a higher number of output keypoints.

%\vspace{-5pt}
\begin{table}[h]
    %\footnotesize
    % \scriptsize
    \begin{center}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c}
    \hline
    Method & Body AP  &	Foot AP \\
    \hline
    % {\scriptsize Body-foot OpenPose++~\cite{cao2018openpose}} & 65.1 & \textbf{25.7} \\
    % {\scriptsize Shallow whole-body++ (ours)} & 60.9 & 21.2 \\
    % {\scriptsize Deep body-foot++ (ours)} & \textbf{65.5} & 21.5 \\
    % {\scriptsize Deep whole-body++ (ours)} & 64.4 & 24.7 \\
    { Body-foot OpenPose (multi-scale)~\cite{cao2018openpose}} & 65.3 & \textbf{77.9} \\
    { Shallow whole-body (ours, multi-scale)} & 60.9 & 70.2 \\
    { Deep body-foot (ours, multi-scale)} & \textbf{66.4} & 76.8 \\
    { Deep whole-body (ours, multi-scale)} & 65.6 & 76.2 \\
    % Method & AP body &	AR body &	AP foot &	AR foot \\
    % \hline
    % {\scriptsize Body-foot OpenPose~\cite{cao2018openpose}} & 65.1 & NA & \textbf{25.7} & \textbf{86.0} \\
    % {\scriptsize Shallow whole-body (ours)} & 60.9 & 67.0 & 21.2 & 83.1 \\
    % {\scriptsize Deep body-foot (ours)} & \textbf{65.5} & \textbf{70.1} & 21.5 & 84.4 \\
    % {\scriptsize Deep whole-body (ours)} & 64.3 & 70.0 & 24.7 & 85.7 \\
    \hline
    \end{tabular}}
    \end{center}
    % \vspace{-10pt}
    \vspace{-5pt}
    \caption{Accuracy results on the COCO
    % and OpenPose-foot validation sets.
    validation set. %Following OpenPose strategy, we apply multi-scale testing for a fair comparison.
    %``AP" refers to Average Precision. % and ``AR" to Average Recall.
    `Shallow' refers to the network architecture with the same depth and input resolution as that of OpenPose, while `Deep' refers to our improved architecture. `Body-foot' refers to the network that simply predicts body and foot keypoints, following the default OpenPose output, while `Whole-body' refers to our novel single-network model.} % that predicts all keypoints at once.}
    % \vspace{-15pt}
    % \vspace{-5pt}
    \label{table:coco_val}
\end{table}

% Table~\ref{table:coco} shows results from top teams in the challenge.



\subsection{Face Keypoint Detection Accuracy}\label{sec:face_val}
In order to evaluate the accuracy of face alignment, traditional approaches have used the Probability of Correct Keypoint (PCK) metric,
%a normalized distance between each keypoint and its ground truth position.
which checks the probability that a predicted keypoint is within a distance threshold of its true location.
However, it %this metric %assumes exactly one face per image.
does not generalize to a multi-person setting.
In order to evaluate our work, we reuse the mean Average Precision (AP) and Recall (AR), following the COCO multi-person metric. % over 10 OKS.
We train our whole-body algorithm with the same face datasets that OpenPose~\cite{cao2018openpose} used: Multi-PIE~\cite{gross2010multi}, FRGC~\cite{frgc_2010}, and i-bug~\cite{sagonas2016300}.
% We create a validation set of about 100 images images out of each one.
We create a custom validation set by selecting a small subset of images from each dataset.
We show the results in Table~\ref{table:face_val}. %of the OpenPose face detector and our approaches. %Note that OpenPose might have been trained with these images already. %, leading to over-fitted results.
We can see that both our method and \cite{cao2018openpose} greatly over-fit on the Multi-PIE and FRGC datasets. These datasets consist of images annotated in controlled lab environments, and all faces appear frontal and with no occlusion, similar to the last image in Fig.~\ref{fig:dataset_examples}. However, their accuracy is considerably lower in the in-the-wild i-bug dataset, where our approach is about 2\% more accurate. %where our approach is considerably better (about 11\%) in the i-bug dataset, which contains in-the-wild images, proving the benefits of multi-task learning for face detection.

%\vspace{-5pt}
\begin{table}[h]
    %\smallsize
    \begin{center}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
    % Method &	AP frgc &	AR frgc & AP MPie &	AR MPie \\
    % \hline
    % {\scriptsize OpenPose~\cite{cao2018openpose}} & 98.3 & 98.9 & \textbf{96.3} & \textbf{96.7} \\
    % {\scriptsize Whole-body, OP arch} & 98.4 & 98.9 & 90.6 & 93.0 \\
    % {\scriptsize Whole-body, new arch} & \textbf{98.4} & \textbf{99.0} & 93.2 & 95.1 \\
    \multirow{2}{*}{ Method } & \multicolumn{3}{c}{Face AR}\\
    \cline{2-4}
    & FRGC & M-Pie & i-bug \\
    \hline
    { OpenPose~\cite{cao2018openpose}} & 98.3 & \textbf{96.3} & 52.4 \\
    { Shallow Whole-body (ours, single-scale)} & \textbf{98.4} & 90.6 & 50.6 \\ %& 55.6 \\
    { Deep Whole-body (ours, single-scale)} & \textbf{98.4} & 93.2 & \textbf{54.5} \\
    % {\scriptsize Shallow whole-body (ours, multi-scale)} & XXX & XXX & XXX \\
    % {\scriptsize Deep whole-body (ours, multi-scale)} & 97.5 & 94.0 & 54.6 \\
    \hline
    \end{tabular}}
    \end{center}
    % \vspace{-10pt}
    \vspace{-5pt}
    \caption{Accuracy results on our custom CMU Multi-PIE and FRGC validation sets. %Note that OpenPose does not implement multi-scale on face detection.
    All the people in each image are not necessarily labeled on i-bug. Thus, those samples might be considered erroneous ``false positives" and affect the AP results. However, AR is only affected by the annotated samples, so it is used as the main metric for i-bug.}
    % \vspace{-15pt}
    % \vspace{-5pt}
    \label{table:face_val}
\end{table}


\subsection{Hand Keypoint Detection Accuracy}\label{sec:hand_val}
% Similarly to the previous annotation tasks, we reuse mean average precision and recall over OKS. We train our hand detector with the two subsets of the OpenPose hand dataset~\cite{simon2017hand}. We denote ``Hand Dome" to the subset recorded in their Panoptic Studio~\cite{Joo_2017_TPAMI}, and ``Hand MPII" to the subset manually annotated from MPII images.
% Once again, 
Analog to face evaluation, we randomly select a subset of images from each hand dataset for validation. We denote ``Hand Dome" for the subset of~\cite{simon2017hand} recorded in the Panoptic Studio~\cite{Joo_2017_TPAMI}, and ``Hand MPII" for the subset manually annotated from MPII~\cite{andriluka14cvpr} images.
% We create a validation set of about 100 images out of each one.
The results are presented in Table~\ref{table:hand_val}. Both our method and the previous OpenPose over-fit on the Dome dataset, where usually only a single person appears in each frame, similar to the first image in Fig.~\ref{fig:dataset_examples}. However, the manually annotated images from MPII are more challenging for both approaches, as it represents realistic in-the-wild scenes. In such images, we can see the clear benefit of our deeper network with respect to Cao~\etal~\cite{cao2018openpose} and our initial shallow model, outperforming by about 5.5\% on the Hand MPII dataset. %, and about 1\% on the Dome dataset. %getting about 5.5\% accuracy improvement, while the improvement in the Dome dataset is only about 2\%. Our approach slightly improves upon OpenPose's accuracy by about 2\% on the Dome dataset, but it highly outperforms it by about 9\% on the MPII dataset. This proves that hand estimation also benefits from multi-task learning.

%\vspace{-5pt}
\begin{table}[b]
    \begin{center}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c}
    \hline
    \multirow{2}{*}{ Method } & \multicolumn{2}{c}{Hand AR}\\
    \cline{2-3}
    & { Dome}  &	{ MPII } \\
    \hline
    { OpenPose (single-scale)~\cite{cao2018openpose}} & 97.0 & 82.7 \\
    { Shallow whole-body (ours, single-scale)} & 94.6 & 82.4 \\
    { Deep whole-body (ours, single-scale)} & \textbf{97.8} & \textbf{88.1} \\
    % {\scriptsize Deep whole-body (ours, multi-scale)} & 94.3 & 78.9  \\
    % Method & AP Dome &	AR Dome &	AP mpii &	AR mpii \\
    % \hline
    % {\scriptsize OpenPose~\cite{cao2018openpose}} & 91.6 & \textbf{97.0} & 73.7 & 82.7 \\
    % {\scriptsize Shallow whole-body} & 91.4 & 94.6 & 73.2 & 82.4 \\
    % {\scriptsize Deep whole-body} & \textbf{93.3} & 95.9 & \textbf{82.8} & \textbf{87.0} \\
    \hline
    \end{tabular}}
    \end{center}
    % \vspace{-10pt}
    \vspace{-5pt}
    \caption{Results on our custom Hand~Dome and Hand~MPII validation sets. These datasets might contain unlabeled people (similar to i-bug), so AR is used for evaluation.}%Note that OpenPose does not implement multi-scale on hand detection.}
    % \vspace{-15pt}
    \label{table:hand_val}
\end{table}


% For camera-ready version
% \subsection{3D Body/POF Keypoint Detection Accuracy}
% \subsection{Car Keypoint Detection Accuracy}




\begin{figure}[t]
% \begin{figure*}[t!] % So figures aligned to top if description texts are too long
\centering
    \includegraphics[width=0.85\linewidth]{figures/runtime_comparison_resized.pdf}
    % \includegraphics[width=.85\linewidth]{figures/runtime_comparison.png}
    \vspace{-5pt}
    \caption{Inference time comparison between our work and whole-body OpenPose~\cite{cao2018openpose}. While the inference time of our proposed approach is invariant, the run-time of OpenPose grows linearly with the number of people.
    OpenPose run-time presents some oscillations because it does not run face and hand detectors if the nose or wrist keypoints (provided by the body network) of a person are not found. This is a common case in images with many crowded images.
    This analysis was performed on a system with a Nvidia 1080 Ti. %, by repeating 1000 times each time measurement. % for each image. %This analysis was performed using the same images for each algorithm and a batch size of 1.
    }
    % \vspace{-12pt}
    % \vspace{-10pt}
\label{fig:runtime_comparison}
\end{figure}





\subsection{Run-time Comparison}\label{sec:runtime_comparison}
In Fig.~\ref{fig:runtime_comparison}, we compare the inference run-time between OpenPose and our work.
Our method is 10\% faster than OpenPose for images with a single person. However, the inference time of our single-network approach remains constant, while OpenPose's time is proportional to the number of people detected, in particular, it is proportional to the number of face and hand proposals. % to be run.
This leads to a massive speedup of our approach
when the number of people increases. For images with $n$ people, our approach is approximately $n$ times faster than OpenPose. For crowded images, many hands and faces are occluded, slightly reducing this speedup.
% OpenPose does not need to run a dedicated network for those candidates.
For instance, our approach is about 7 times faster than OpenPose for typical images with 10 people in them.
% our method have a constant inference run-time, opposite to OpenPose, leading to $\times2$ speedup for 2-people images, $\times3$ for 3-people images, or about $\times7$ in 10-people images.
% The analysis is performed on images with various amounts of people, only measuring the time spent on the network and person parsing algorithm. % (excluded image reading, resize to the network resolution, and display),
% and it is repeated 1000 times.
% The run-time of our approach consists of the CNN network processing time, with complexity $O(1)$, and the multi-person parsing time, with complexity is $O(p^2)$, where $n$ is the number of people. However, the parsing time is about two orders of magnitude smaller than the network time.



% \section{Failure Case Analysis}
% We analyze the cases where our approach recursively fails. Fig.~\ref{fig:failure_examples} shows an overview of those. Fig.~\ref{fig:failure_examples}a refers to non typical poses and upside-down examples, where the predictions usually fail. Increasing the rotation augmentation visually seems to partially solve these issues, but the global accuracy would be reduced, as shown in~\cite{cao2018openpose}. Body occlusion can also lead to false negatives and high localization error. This problem is inherited from the dataset annotations, in which occluded keypoints are not included. In highly crowded images where people are overlapping, the approach tends to merge annotations from different people, while missing others, due to the overlapping PAFs that make the greedy multi-person parsing fail. Animals and statues also frequently lead to false positive errors. This issue could be mitigated by adding more negative examples during training to help the network distinguish between humans and other humanoid figures.


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/5_conclusion.tex <==
\section{Conclusion}
In this paper, we resort to multi-task learning combined with an improved model architecture to train the first single-network approach for 2D whole-body estimation. % Analogous to what Fast R-CNN did for object detection, 
Our work brings together multiple and, currently, independent keypoint detection tasks into a unified framework.
% Our method combines different datasets with different keypoint characteristics into a single network.
% While most traditional multi-task learning methods iteratively expose their network to a fixed number of epochs for each dataset, we train our model in a single shot, by randomly sampling annotations from each dataset.
We evaluate our method on multiple keypoint detection benchmarks and compare it with the state-of-the-art, considerably outperforming it in both training and testing speed as well as slightly improving its accuracy. %Body-only detection accuracy is maintained similar. %, while maintaining a similar body detection accuracy.
% We also achieve very competitive results for body estimation in COCO and MPII challenges, comparable with the start-of-the-art. In addition, w
We qualitatively show in Fig.~\ref{fig:qualitative_results} that our face and hand detectors generalize better to in-the-wild images, % compared to those of OpenPose,
benefiting from their indirect exposure to the immense body datasets. %given that their backbone has been also exposed to the massive body pose datasets.
Nevertheless, there are still some limitations with our method. First, we observe global failure cases when a significant part of the target person is occluded or outside of the image boundaries. Secondly, the accuracy of the face and especially hand keypoint detectors is still limited, failing in the case of severe motion blur, small people, and extreme gestures. %Our approach to jointly train tasks from different datasets could be potentially extended / leverage the computation required for any real-world application that require similar but different algorithms to run. %For instance, 2D and 3D human keypoint estimation could be combined into a single approach, potentially helping the 3D detector benefit from the robust 2D datasets.
Third, we qualitatively observe that the previous version of OpenPose outperforms ours for face and hand detection when poses are simple and no occlusion occurs. The previous method crops the bounding box proposal of those bounding box candidates, resizes them up, and feeds them into its dedicated networks. This higher input resolution leads to an increased pixel localization precision if the keypoint detection is successful.
%We will publicly release the code, trained models, and validation benchmark as a baseline for future work in whole-body pose estimation.


==> ICCV 2019 - Post Camera Ready (Arxiv) - Single-Network Whole-Body Pose Estimation/section/6_qualitative_results.tex <==
\begin{figure*}[ht]
\centering
    \begin{subfigure}[t]{1.\textwidth}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000001841_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000002116_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/luka_doncic_000000004441_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/luka_doncic_000000000563_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000001235_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}[t]{1.\textwidth}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/selfie_000000000280_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000000424_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000001808_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000001731_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/good/live_it_up_000000002310_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}[t]{1.\textwidth}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/fail/luka_doncic_000000000992_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/fail/live_it_up_000000002053_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/fail/live_it_up_000000000880_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/fail/hillary_vs_trump_000000000252_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
        \begin{subfigure}[t]{0.195\textwidth}
        \includegraphics[width=1\linewidth]{figures/fail/luka_doncic_000000000918_rendered.jpg}
        \vspace{-17.5pt}
        \caption{}
        \end{subfigure}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Qualitative comparison between our method (top) and the previous version of OpenPose~\cite{cao2018openpose} (bottom), performed on a system with 2 Nvidia 1080 Ti.
    (a-j)~show improved results and (k-o) failing cases.
    (a)~It generalizes better to hands wearing any kind of gloves.
    (b)~The implicit finger information helps wrist and elbow detection.
    (c)~Even smaller faces and hands are detected.
    (d-e)~Blurry and profile faces are detected.
    (f)~More extreme hand poses are detected.
    (g)~Faces from low-brightness images are better detected.
    (h)~Hands where all fingers are occluded are detected.
    (i-j)~Cropped arms are properly detected.
    (k-l)~It shows difficulties when several hands are in proximity.
    % (m-o)~It seems to fail for some relatively easy hand and face poses for which OpenPose detection works.
    (m-o)~It seems to fail for some relatively easy hand and face poses that are successfully detected with the previous version of OpenPose.
    % Our approach considerably outperforms OpenPose in speed, and it is able to detect a higher number of faces and hands. It is particular better on blurry face/hands as well as hands wearing gloves.
    }\label{fig:qualitative_results}
%   \caption{Qualitative comparison between our method and OpenPose.}
    % \vspace{-10pt}
% \label{fig:failure_examples}
\end{figure*}


==> section/0_teaser.tex <==
% \begin{figure}[t]
%     \centering
    \includegraphics[width=1\linewidth]{figures/teaser/teaser_final.jpg}
    % \begin{subfigure}[t]{1\textwidth}
    % \begin{subfigure}[t]{0.499\textwidth}
    % \includegraphics[width=1\linewidth]{figures/teaser/teaser_OP.png}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.499\textwidth}
    % \includegraphics[width=1\linewidth]{figures/teaser/teaser_our.png}
    % \end{subfigure}
    % \end{subfigure}
    \captionof{figure}{We present the first single-network approach for whole-body pose estimation, with real-time performance independent of the number of people in the image. Our work builds upon the current state-of-the-art OpenPose~\cite{cao2018openpose}, boosting considerably its run-time performance while simultaneously improving slightly on the keypoint accuracy.} \label{fig:teaser}
% \end{figure}

